Spiral of Silence: How is Large Language Model Killing Information Retrieval? -- A Case Study on Open Domain Question Answering

The practice of Retrieval-Augmented Generation (RAG), which integrates Large Language Models (LLMs) with retrieval systems, has become increasingly prevalent. However, the repercussions of LLM-derived content infiltrating the web and influencing the retrieval-generation feedback loop are largely uncharted territories. In this study, we construct and iteratively run a simulation pipeline to deeply investigate the short-term and long-term effects of LLM text on RAG systems. Taking the trending Open Domain Question Answering (ODQA) task as a point of entry, our findings reveal a potential digital "Spiral of Silence" effect, with LLM-generated text consistently outperforming human-authored content in search rankings, thereby diminishing the presence and impact of human contributions online. This trend risks creating an imbalanced information ecosystem, where the unchecked proliferation of erroneous LLM-generated content may result in the marginalization of accurate information. We urge the academic community to take heed of this potential issue, ensuring a diverse and authentic digital information landscape.

==> parts/tables/chinese_bleu.tex <==
{\setlength{\belowcaptionskip}{-4pt}
\begin{figure*}[h]
  \centering
  % \setlength{\belowcaptionskip}{-0.1cm}
  \begin{subfigure}[t]{0.21\textwidth}
    \includegraphics[width=\textwidth]{images/chinese_plot_nq_tsv.png}
    \caption{NQ}
    \label{fig:chinese_nq_bleu}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.21\textwidth}
    \includegraphics[width=\textwidth]{images/chinese_plot_webq_tsv.png}
    \caption{WebQ}
    \label{fig:chinese_webq_bleu}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.21\textwidth}
    \includegraphics[width=\textwidth]{images/chinese_plot_tqa_tsv.png}
    \caption{TriviaQA}
    \label{fig:chinese_tqa_bleu}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.31\textwidth}
    \includegraphics[width=\textwidth]{images/chinese_plot_pop_tsv.png}
    \caption{PopQA}
    \label{fig:chinese_pop_bleu}
  \end{subfigure}
  \caption{3-gram Self-BLEU score for the top 5 search results over iterations, from the original dataset (Ori.) to the inclusion and subsequent iterations with LLM-generated texts. 
  %We only present the results on NQ and PopQA; 
  For results on WebQ and TriviaQA, please refer to Figure~\ref{fig:BLEU_app} in Appendix~\ref{sec:app_fig_wt}.}
  \label{fig:chinese_BLEU}
\end{figure*}}

==> parts/tables/short-term-back.tex <==
\begin{table*}[htbp]
\centering
\caption{Differences between acc@5 origin}
\resizebox{1\textwidth}{!}{
\begin{tabular}{l|ll|ll|ll|ll}
\toprule
\multirow{2}{*}{acc@5} & \multicolumn{2}{c|}{NQ} & \multicolumn{2}{c|}{WebQ} &  \multicolumn{2}{c|}{TriviaQA}&\multicolumn{2}{c}{PopQA}  \\
\cline{2-9}
& origin & loop1 & origin & loop1 &  origin & loop1 &origin & loop1 \\
\toprule
BM25                  & 49.0   & \ApplyGradient{49.0}{57.5} & 41.0   & \ApplyGradient{41.0}{51.0}$^*$  &  62.5   & \ApplyGradient{62.5}{82.0}$^*$  &35.5   & \ApplyGradient{35.5}{41.5} \\
Contreiver            & 68.0   & \ApplyGradient{68.0}{68.5} & 66.0   & \ApplyGradient{66.0}{69.5} &  68.0   & \ApplyGradient{68.0}{83.5}$^*$ &62.0   & \ApplyGradient{62.0}{65.0}  \\
LLM-embedder          & 75.5  & \ApplyGradient{75.5}{75.5} & 62.5  & \ApplyGradient{62.5}{72.5}$^*$ &  67.5  & \ApplyGradient{67.5}{81.0}$^*$  &70.0    & \ApplyGradient{70.0}{67.5} \\
BGE-base              & 77.0   & \ApplyGradient{77.0}{73.0}  & 65.5  & \ApplyGradient{65.5}{71.5} &  69.5  & \ApplyGradient{69.5}{81.5}$^*$ &72.0   & \ApplyGradient{72.0}{70.0}   \\
BM25+UPR              & 63.0   & \ApplyGradient{63.0}{66.5}  & 57.0   & \ApplyGradient{57.0}{68.0}$^*$  &  71.5  & \ApplyGradient{71.5}{83.0}$^*$  &57.5  & \ApplyGradient{57.5}{61.5} \\
BM25+MonoT5           & 66.5  & \ApplyGradient{66.5}{69.0}  & 62.0   & \ApplyGradient{62.0}{67.5} &  72.0   & \ApplyGradient{72.0}{83.5}$^*$ &53.5  & \ApplyGradient{53.5}{58.5} \\
BM25+BGE-reranker     & 68.0   & \ApplyGradient{68.0}{69.5}  & 64.5  & \ApplyGradient{64.5}{68.5} &  72.5  & \ApplyGradient{72.5}{84.0}$^*$  &54.0   & \ApplyGradient{54.0}{61.0}  \\
BGE-base+UPR          & 75.5  & \ApplyGradient{75.5}{71.5}  & 64.0   & \ApplyGradient{64.0}{69.0}  &  76.0   & \ApplyGradient{76.0}{84.0}$^*$  &76.0   & \ApplyGradient{76.0}{71.0}  \\
BGE-base+MonoT5       & 75.0   & \ApplyGradient{75.0}{70.5}  & 68.5  & \ApplyGradient{68.5}{72.0}  &  77.0   & \ApplyGradient{77.0}{83.5} &72.0   & \ApplyGradient{72.0}{72.5} \\
BGE-base+BGE-reranker & 69.0   & \ApplyGradient{69.0}{68.0}  & 67.5  & \ApplyGradient{67.5}{70.5} &  72.5  & \ApplyGradient{72.5}{83.5}$^*$ &73.0   & \ApplyGradient{73.0}{70.0}   \\
\bottomrule
\end{tabular}}
\label{tab:short_ret}
\end{table*}


\begin{table*}[htbp]
\centering
\caption{Differences between acc@20 origin}
\resizebox{1\textwidth}{!}{
\begin{tabular}{l|ll|ll|ll|ll}
\toprule
\multirow{2}{*}{acc@20} & \multicolumn{2}{c|}{NQ} & \multicolumn{2}{c|}{WebQ} &  \multicolumn{2}{c|}{TriviaQA}&\multicolumn{2}{c}{PopQA}  \\
\cline{2-9}
& origin & loop1 & origin & loop1 &  origin & loop1 &origin & loop1 \\
\toprule
BM25                  & 67.0 & \ApplyGradient{67.0}{73.5} & 63.0 & \ApplyGradient{63.0}{71.0}  &  73.0 & \ApplyGradient{73.0}{87.0}$^*$  &51.5 & \ApplyGradient{51.5}{59.5} \\
Contreiver            & 84.0 & \ApplyGradient{84.0}{85.0} & 74.0 & \ApplyGradient{74.0}{80.0} &  80.5 & \ApplyGradient{80.5}{87.5} &77.5 & \ApplyGradient{77.5}{79.5}  \\
LLM-embedder          & 86.5 & \ApplyGradient{86.5}{88.0} & 76.0 & \ApplyGradient{76.0}{79.5} &  77.5 & \ApplyGradient{77.5}{87.5}$^*$  &79.5 & \ApplyGradient{79.5}{82.0} \\
BGE-base              & 86.0 & \ApplyGradient{86.0}{86.0}  & 77.0 & \ApplyGradient{77.0}{80.0} &  80.0 & \ApplyGradient{80.0}{87.5}$^*$ &83.0 & \ApplyGradient{83.0}{84.5}   \\
BM25+UPR              & 73.5 & \ApplyGradient{73.5}{78.0}  & 68.5 & \ApplyGradient{68.5}{75.0}  &  78.0 & \ApplyGradient{78.0}{89.0}$^*$  &60.0 & \ApplyGradient{60.0}{67.0} \\
BM25+MonoT5           & 74.5 & \ApplyGradient{74.5}{80.5}  & 69.5 & \ApplyGradient{69.5}{76.0} &  78.0 & \ApplyGradient{78.0}{88.0}$^*$ &59.5 & \ApplyGradient{59.5}{66.5} \\
BM25+BGE-reranker     & 76.5 & \ApplyGradient{76.5}{81.0}  & 71.0 & \ApplyGradient{71.0}{76.0} &  78.0 & \ApplyGradient{78.0}{88.5}$^*$  &60.0 & \ApplyGradient{60.0}{67.5}  \\
BGE-base+UPR          & 87.5 & \ApplyGradient{87.5}{88.0}  & 77.0 & \ApplyGradient{77.0}{79.5}  &  84.5 & \ApplyGradient{84.5}{89.5}  &84.5 & \ApplyGradient{84.5}{84.5}  \\
BGE-base+MonoT5       & 86.5 & \ApplyGradient{86.5}{86.5}  & 78.0 & \ApplyGradient{78.0}{81.5}  &  83.5 & \ApplyGradient{83.5}{89.5} &85.5 & \ApplyGradient{85.5}{86.0} \\
BGE-base+BGE-reranker & 84.0 & \ApplyGradient{84.0}{84.5}  & 78.0 & \ApplyGradient{78.0}{81.5} &  82.0 & \ApplyGradient{82.0}{88.0} &84.0 & \ApplyGradient{84.0}{85.0}   \\
\bottomrule
\end{tabular}}
\label{tab:short_ret}
\end{table*}

==> parts/tables/short_term_figure.tex <==
\begin{figure*}[htbp]
  \centering
  \setlength{\belowcaptionskip}{-0.4cm}
  \begin{subfigure}[t]{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/nq.png}
    \caption{figure1}
    \label{fig:image1}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/webq.png}
    \caption{figure2}
    \label{fig:image2}
  \end{subfigure}
  
  \vspace{0.2cm}
  
  \begin{subfigure}[t]{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/tqa.png}
    \caption{figure3}
    \label{fig:image3}
  \end{subfigure}
  \hfill
  \begin{subfigure}[t]{0.49\textwidth}
    \centering
    \includegraphics[width=\textwidth]{images/pop.png}
    \caption{figure4}
    \label{fig:image4}
  \end{subfigure}

  \caption{figures}
  \label{fig:subfigures}
\end{figure*}
